BEBERT: Efficient and Robust Binary Ensemble BERT

Pre-trained BERT models have achieved impressive accuracy on natural language processing (NLP) tasks. However, their excessive amount of parameters hinders them from efficient deployment on edge devices. Binarization of the BERT models can significantly alleviate this issue but comes with a severe accuracy drop compared with their full-precision counterparts. In this paper, we propose an efficient and robust binary ensemble BERT (BEBERT) to bridge the accuracy gap. To the best of our knowledge, this is the first work employing ensemble techniques on binary BERTs, yielding BEBERT, which achieves superior accuracy while retaining computational efficiency. Furthermore, we remove the knowledge distillation procedures during ensemble to speed up the training process without compromising accuracy. Experimental results on the GLUE benchmark show that the proposed BEBERT significantly outperforms the existing binary BERT models in accuracy and robustness with a 2x speedup on training time. Moreover, our BEBERT has only a negligible accuracy loss of 0.3% compared to the full-precision baseline while saving 15x and 13x in FLOPs and model size, respectively. In addition, BEBERT also outperforms other compressed BERTs in accuracy by up to 6.7%.

==> 0-abstr.tex <==
\begin{abstract}

Despite the achievement of pre-trained models in natural language processing(NLP) tasks, the enormous number of parameters and excessive storage costs pose difficulties for deployment on edge devices.
To tackle the challenges, model compression strategies based on model quantization could compress the model proportionally, especially quantizing the parameters to 1 bit could yield stunning results. 
Nevertheless, the performance of existing binarization models still falls short compared to the full-precision counterparts; in particular, there is an accuracy gap on small datasets. 
To solve this problem, we suggest a new compression paradigm for developing efficient and robust binary BERTs for real-time deployment, boosting accuracy and stability while maintaining model efficiency.
The proposed BEBERT in this paper develops hardware-efficient networks by adopting the ensemble learning approach for multiple binary models and also realizes time-efficient training via simplifying the knowledge distillation(KD) process. Experimental results show that our BEBERT achieves the best results among the state-of-the-art binary BERT models on various tasks in the GLUE dataset and surpasses the existing compressed full-precision BERTs, with up to \textbf{15x} and \textbf{13x} saving on FLOPs and model size.
\end{abstract}

==> 1-intro.tex <==
\section{Introduction}

Pre-trained BERT models (e.g., BERT\cite{devlin2019bert}, RoBERTa\cite{liu2019roberta}, Xlnet\cite{yang2019xlnet}) provide significant accuracy improvement to many natural language processing (NLP) tasks. However, deploying them on resource-limited devices is difficult due to the massive amount of parameters and expensive storage costs. 
To tackle this challenge, model compression techniques, including quantization\cite{zafrir2019q8bert}\cite{shen2020q}, pruning\cite{chen2021earlybert}\cite{hou2020dynabert}, and distillation\cite{jiao2020tinybert}\cite{sun2020mobilebert}, are widely studied and applied to promote employing BERT models in resource-constrained and real-time scenarios.

Among these model compression methods, quantization has been an attractive method since it can significantly reduce the model size and computational intensity by simply reducing the bit width of the parameters without changing the models' architecture. 
The most aggressive quantization scheme, dubbed as binarization(for example, in \cite{bai2021binarybert} and \cite{qin2022bibert}), allows the BERT models to utilize 1-bit parameters and efficient bitwise operations, which can significantly reduce the storage consumption and inference cost. 
However, experiments show that the existing works produce severe accuracy degradation problems compared to full precision models on GLUE datasets. Especially for tiny datasets, \cite{bai2021binarybert} faces an 11.3\% decrease in CoLA dataset and \cite{qin2022bibert} even does not attain half of the accuracy.

In this paper, we propose BEBERT, an optimized binary BERT model based on the ensemble learning\cite{dietterich2000ensemble} methods, which can apply to both weight-binarized and fully-binarized BERT models and attain appealing accuracy improvement. 
Specifically, to substantiate the universality for ensemble methods in BERT, we use BiBERT and BinaryBERT as the backbone models, respectively, and obtain an average accuracy improvement of \textbf{2.7\%} and  \textbf{4.0\%}. 
The extensive experiments on the GLUE\cite{wang2018glue} benchmark show that our BEBERT based on BinaryBERT outperforms existing full-precision compressed BERTs by \textbf{1\%-4\%}, with a notable \textbf{15x} and \textbf{13x} saving on FLOPs and model size, which contributes to hardware-efficient advantages.
Furthermore, we simplify the KD process during training without accuracy reduction to realize a time-efficient training process.
% BEBERT reserves the two advantages of the binary models: proportional reduction of the number of parameters and replacing floating-point units with bit-operation. 
The main contributions of this paper can summarize as follows: 
1) We indicate that ensemble learning techniques benefit binary BERT models for bridging the performance gap between binary BERTs and their full-precision counterparts. 
2) We introduce BEBERT, an efficient and robust binary BERT model, which outperforms the state-of-the-art full-precision compressed BERTs, providing an accurate and hardware-efficient approach for real-time BERT deployment.
3) We achieve time-efficient training by simplifying the training process, with discussion on whether KD approachs are needed during ensemble learning with different base learners.






==> 2-rel.tex <==
\section{Related Works} \label{sec:rel}

% \begin{figure*}[htbp]  
% \centering  
% \subfloat[Structures of BEBERTs based on BinaryBERT.]{  \label{fig:1}  
% \begin{minipage}[t]{0.42\textwidth}  
% \centering  
% \includegraphics[width=\linewidth,scale=1.00]{./figs/BEBERT_mod.png}
% \end{minipage}  }
% \subfloat[Structures of BEBERTs based on BiBERT.]{  
% \label{fig:2}  
% \begin{minipage}[t]{0.42\textwidth}  
% \centering  
% \includegraphics[width=\linewidth,scale=1.00]{./figs/BEBERT3_mod.png}
% \end{minipage}  }
% \caption{Structures of BEBERT: The color of lines represents different KD methods.}  
% \end{figure*}

\begin{figure}[htbp]  
\centering  
\label{fig:1}  
\centering  
\includegraphics[width=\linewidth,scale=1.00]{./figs/BEBERT.png}
\caption{Structure of BEBERT(BinaryBERT-based): The color of lines represents different KD methods.}  
\end{figure}

\textbf{Quantization} is one of the important means of model compression, and so far, it has been widely used in Transformer-based models\cite{kim2021bert}\cite{zadeh2020gobo}. 
Extreme quantization\cite{bai2021binarybert}\cite{qin2022bibert} methods, with binarized parameters, can replace floating-point operations with bit operations and is able to achieve $O(1)$ operational complexity. 
Accordingly, the speed, storage, and power advantages of BNNs bring new momentum to the deployment of large pre-trained models in edge devices. 
However, obtaining model parameters with a bit-width of 1 is accompanied by a significant loss of accuracy. 
% To address the problem of improving BNNs' accuracy, researchers have proposed a series of optimization methods, such as  divided into three main categories. For instance, \cite{ courbariaux2015binaryconnect}\cite{rastegari2016xnor} introduces a scaling factor $\alpha$ to minimize quantization error;  \cite{polino2018model}, and others innovated the loss function using distillation methods; 
% \cite{bengio2013estimating} promoted the STE method for gradient estimation in the binarization backpropagation process.
Based on the existing BNNs' optimization methods, the BEBERT put forward in this paper further approximates the performance of BNN and full-precision models at the cost of operational complexity increases to O(N).

\noindent\textbf{Ensemble learning} includes a variety of machine learning algorithms that integrate the predictions of N weak classifiers using multiple voting mechanisms to improve classification accuracy. 
% Typical integrated learning algorithms for classification models include bagging\cite{breiman1996bagging} and boosting\cite{freund1996experiments}, the latter has several derivation as AdaBoost\cite{freund1997decision}, GBDT\cite {friedman2002stochastic}, etc. 
% Although bagging is beneficial to improve inference speed, as each model trains independently, it is an elementary method with plain performance. 
Among the ensemble techniques,  boosting\cite{freund1996experiments}\cite{freund1997decision} achieves great performance in various tasks, and it is first applied to deep neural networks by \cite{schwenk2000boosting}. 
% The main theory of boosting algorithm is to adjust the weights of the samples continuously during training based on the prediction error of the previous weak learner and trains the next model serially, which can usually attain better performance. 
Recently, researchers have used ensemble techniques to improve the performance of neural networks, such as \cite{moghimi2016boosted} and \cite{BAIG2017120}, and constantly achieve desirable results. Inspired by the success of boosting techniques in past works, we apply them to binary BERTs. The results show that our BEBERTs based on BinaryBERT can consistently achieve better performance when the number of boosting iterations equals 2. We also compare the accuracy to several full-precision compression models and find that the AdaBoost-based BEBERT we introduced always has the advantage in accuracy with a reduced operational complexity from $\frac{O(32^2)}{K}$ to $O(N)$.

\noindent\textbf{Knowledge distillation} is a model compression method designed for reducing the size of pre-trained models, which is firstly used in the NLP area by \cite{hinton2015distilling}. 
KD enhances the generalization ability of student models by transferring the knowledge learned from large teacher models to light student models. 
Many recent works\cite{jiao2020tinybert}\cite{sun2020mobilebert}\cite{wang2020minilm} have designed different objective functions for improving the KD BERT. 
For instance, logits/predictions, embedding layer outputs, self-attention distributions, and hidden states of each Transformer layer are used as the KD objects.
In this work, we explore the performance of ensemble binary BERT under KD-free and KD with different objective functions. That way, we could verify the ensemble approach's dependence on KD methods for simplifying the training process.

%%----------------------------------------------------------------
%以前那版，强调了QNN<BNN,但是文中没有最后和QNN比较，遂进行了修改
%%----------------------------------------------------------------
% \textbf{Quantization} is one of the important means of model compression, and so far, it has been widely used in Transformer-based models. However, for the k-bit fixed-point quantization models\cite{zafrir2019q8bert}\cite{kim2021bert}, whose operational complexity is $O(K^2)$; although the state-of-the-art has attained similar performance as the full-precision ones, cannot realize the inference process of bit-wise operations. Nevertheless, binary quantization\cite{bai2020binarybert}\cite{qin2022bibert} methods, which can replace floating-point operations with bit operations, is able to achieve $O(1)$ operational complexity. Accordingly, the speed, storage, and power advantages of BNNs bring new momentum to the deployment of large pre-trained models in edge devices. However, obtaining model parameters with a bit-width of 1 is accompanied by a significant loss of accuracy. To address the problem of improving BNNs' accuracy, researchers have proposed a series of optimization methods divided into three main categories: minimize quantization error, improve loss function, and reduce gradient error. \cite{ courbariaux2015binaryconnect} \cite{rastegari2016xnor} introduces a scaling factor $\alpha$ to bridge the gap between the binarization parameter and the full precision value; \cite{hou2016loss} pioneers the innovative loss function to reduce the loss during training, \cite{polino2018model}, and others innovated the loss function using distillation methods; \cite{bengio2013estimating} promoted the STE method for gradient estimation in the binarization backpropagation process. Based on the existing BNNs' optimization methods, the BEBERT put forward in this paper further approximates the performance of BNN and full-precision models at the cost of operational complexity increases to O(N).

==> 3-algo.tex <==
\section{Methods} \label{sec:methods}

\subsection{Model Architecture}
As shown in Fig. \ref{fig:1}, we use BinaryBERT and BiBERT as the backbone models for ensemble, respectively. Additionally, we simplify the distillation methods in the training process of BEBERT while maintaining the performance simultaneously.

\subsection{Training BEBERT with ensemble}
\label{sec:ensemble-learning}
To bridge the performance gap between binary models and their full-precision counterparts, AdaBoost is used to integrate binary BERTs to build our efficient and robust BEBERT. 
The detailed training process is shown in Algorithm~\ref{agr: 1}.

There are many derivations of boosting algorithms, and the reason for choosing the emblematic AdaBoost to increase the efficiency and robustness of binary BERTs is as follows. 
% The principle of boosting algorithm is to continuously adjust the sample weights during training based on the prediction error of the previous weak learner and train the next model serially.
As \cite{qin2022bibert} mentioned, binary models are prone to distillation direction mismatch problems, so we abandon the boosting algorithms that reweight on gradient or loss and choose AdaBoost based on sample weights' reweighting to decrease the probability of optimization mismatch.
% Eventually, BEBERT with AdaBoost shows evident improvement in binary BERT models' accuracy and robustness and exceeds numerous state-of-the-art full-precision models.


\begin{algorithm}[htbp]
\caption{Training BEBERT with ensemble} %算法的名字
\label{agr: 1}
\begin{algorithmic}[1]
\State \textbf{Initialize:} $m$ examples $\langle(x_1, y_1),...,(x_m,y_m)\rangle$ in the training set; $y_j\in Y$ represents the labels and $D_1=(w_{11}...w_{1m})=(\frac{1}{m}...\frac{1}{m})$ is the sample weight;
\State \textbf{Input:} training set with sample weights $D_1$;
\For{$i = 1$ to $N$}
    \For{$iter = 1$ to $T$} % For 语句，需要和EndFor对应
        \State Get next mini-batch of training data;
        \State Binarize $w$ in student model to $w_b$;
        \If {KD} % If 语句，需要和EndIf对应
            \State Compute distillation loss between $h^T$ and $h_i^S$;
        \Else
            \State Compute loss between $Y$ and $h_i^S$;
        \EndIf
        \State Backward propagation to compute the gradients;
        \State Update weights with the gradients $\frac{\partial L}{\partial w_b}$;
    \EndFor
    \State Calculate the error $e_i$ and weight $\alpha_i$ of $h_i^S$; % in equation\ref{eqa:1}
    \State Update the sample weight $D_{i+1}$; % in equation\ref{eqa:2}
\EndFor
\State \textbf{Output:} The final hypothesis $H\leftarrow \Sigma_{i=1}^N\alpha_i h_i(x_i)$; % in equation\ref{eqa:3}
\end{algorithmic}
\end{algorithm}

\subsection{Finetuning BEBERT with various KD methods}
\label{sec: KD}
KD is a classic approach to strengthen the generalization ability for small-scale student models, which has extensive use in the NLP area. 
To alleviate performance decrease in binary BERTs, we incorporate the KD technique in each finetuning process to improve the efficiency and robustness of our BEBERT.
Moreover, we design diverse objective functions for distillation to simplify the training process.

Specifically, inspired by \cite{jiao2020tinybert}, the
distillation objective consists of three parts in the first stage, which calculates the embedding, attention, and hidden loss. And in the second stage, we extract knowledge from the prediction layer. The representation for the loss functions are:
\begin{equation}
    \footnotesize
    L_{trm}=\Sigma_{l=1}^{L+1}MSE(H_l^T, H_l^S)+\Sigma_{l=1}^{L}MSE(A_l^T, A_l^S),
\end{equation}
\begin{equation}
    \small
    L_{pred}=SCE(P^T, P^S),
\end{equation}
where $H_l^T, P^T, A_l^T$ represent the hidden states, prediction layer outputs, and attention matrix of teacher networks, and $H_l^S, P^S, A_l^S$ refer to their counterpart in the student networks.
$MSE$ means the mean squared error loss function, and $SCE$ means the soft cross-entropy loss function. $l$ means the number of the layer, $L=12$.

\begin{figure}[htbp]  
\centering  
\subfloat[CoLA]{  
\centering  
\includegraphics[width=\linewidth]{./figs/CoLA.png}} \\
\subfloat[SST-2]{  
\centering  
\includegraphics[width=\linewidth]{./figs/SST2.png}}  
\caption{Ablation study for BEBERT with different KD methods. \textbf{Left}: ensemble BinaryBERT training with three kinds of KD methods compared with the origin. \textbf{Right}: ensemble BiBERT} 
\label{fig:3} 
\end{figure}

% We observe more distinctive effects of our BEBERTs than regular networks. To verify this point, 
For ensemble BinaryBERT, we compare the results when integrating with prediction KD, two-stage KD, and without KD. 
% Specifically, the base learner of BEBERT with KD in the prediction layer is a half-trained binary model finetuned by the first KD stage distillation. 
Moreover, we also measure BiBERT w and w/o KD during training and then analyze the performances. 
Results show that whether to apply KD in ensemble BinaryBERT(left pictures in Fig. \ref{fig:3}) has a minor effect on its behavior in each dataset. However, the ablation experiment shows a sharp drop in accuracy when detaching the KD method from the training process of ensemble BiBERT(right pictures in Fig. \ref{fig:3}) in several GLUE datasets. 

One explanation is that the performance of the base learner determines the effect of KD methods. Since BiBERT is a fully binarized model with a comparably worse capacity for inference, so the KD process is necessary to maintain its expected behavior during ensemble. On the contrary, integrating a stronger learner w/o KD efficiently saves training time and preserves similar lift on results.

% Boosting can reduce the bias of weak learners and optimize them with a stage-wise gradient descent method. 
% Take AdaBoost for instance, suppose there are $m$ examples in the training set, we firstly initialize the weight distribution as: $D_1=(w_{11}...w_{1m})=(\frac{1}{m}...\frac{1}{m})$. In the $i^{th}$ iteration, the weak learner $ h_i$'s sample weights are updated by increasing the weights of error prediction, and the model weight $\alpha_i$ is assigned for $h_i$. Accordingly, we obtain the final prediction by voting based on the classifiers' weights $\alpha$. Suppose the input is $x_i$, the label for the training set is $y_i$, and the output error and model weights for the classifier $h_i$ formulate as Equation \ref{eqa:1}. Equation \ref{eqa:2} indicates the iteration function for the sample weights, and Equation \ref{eqa:3} represents the strong classifier composed of N weak ones.
% \begin{equation}
% \label{eqa:1}
% \small
% \begin{aligned}
%     e_i=P(h_i(x_i)\neq y_i)&=\frac{\Sigma_{j=1}^m w_{ij}I(h_i(x_{ij})\neq y_{ij})}{\Sigma_{j=1}^m w_{ij}}\\\alpha_i&=\frac{1}{2}ln\frac{1-e_i}{e_i}
% \end{aligned}
% \end{equation}
% \begin{equation}
% \small
% \label{eqa:2}
%     D_{i+1}(j) = D_i(j)\exp(-\alpha_i y_{ij} h_i(x_{ij}))
% \end{equation}
% \begin{equation}
% \small
% \label{eqa:3}
%     H=\Sigma_{i=1}^N\alpha_i h_i(x_i)
% \end{equation}


==> 4-res.tex <==
% \begin{table*}[htbp]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|lll|l||lllllll|l}
% \hline
% \textbf{Method}  & \textbf{\#Bits} & \textbf{Size(MB)} & \textbf{FLOPs} & \textbf{DA} & \textbf{MNLI-mm} & \textbf{QQP}  & \textbf{QNLI}  & \textbf{SST-2} & \textbf{CoLA} & \textbf{MRPC} & \textbf{RTE}  & \textbf{Avg.}    \\ \hline
% \textbf{BEBERT$_{\text{using }\cite{qin2022bibert}}$} & 1-1-1           & 13.4n        & 0.4          & \XSolidBrush           & \textbf{76.6}    & \textbf{84.9} & \textbf{80.7}  & \textbf{90.2}  & \textbf{27.7} & \textbf{75.1} & \textbf{58.6} & \textbf{70.54} \\
% \textbf{BiBERT \cite{qin2022bibert}} & 1-1-1           & 13.4          & 0.4            & \XSolidBrush           & 67.5             & 84.8          & 72.6           & 88.7           & 25.4          & 72.5          & 57.4          & 66.99        \\ \hline
% \textbf{BEBERT} & 1-1-1           & 13.4n        & 0.4          & \Checkmark           & \textbf{76.6}    & \textbf{84.9} & \textbf{80.7*} & \textbf{91.8}  & \textbf{42.6} & \textbf{82.4} & \textbf{65.8} & \textbf{74.97} \\
% \textbf{BiBERT} & 1-1-1           & 13.4          & 0.4            & \Checkmark           & 67.5             & 84.8          & 76             & 90.9           & 37.8          & 78.8          & 61            & 70.97         \\ \hline
% \end{tabular}
% }
% \caption{Results on the GLUE development set for ensemble BiBERT(n=8).}
% \label{table:1}
% \end{table*}

% \begin{table*}[htbp]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|lll|l|l||lllllll|l}
% \hline
% \textbf{Method}                   & \textbf{\#Bits} & \textbf{Size} & \textbf{FLOPs} & \textbf{KD} & \textbf{DA} & \textbf{MNLI-mm} & \textbf{QQP}   & \textbf{QNLI} & \textbf{SST-2} & \textbf{CoLA} & \textbf{MRPC} & \textbf{RTE}  & \textbf{Avg.}  \\ \hline
% {\textbf{BEBERT}} & 1-1-4           & 33(x12.7)     & 1.5            & \textbf{A}  & \XSolidBrush  & 84.6   & \textbf{91.2*} & \textbf{91.2} & \textbf{93.3}  & 54.4          & \textbf{86.5} & 68.8          & 81.43          \\
%                                  & 1-1-4           & 33(x12.7)     & 1.5            & \textbf{B}  & \XSolidBrush  & \textbf{84.8}    & 91.2 & \textbf{91.2} & \textbf{93.3}  & \textbf{54.8} & \textbf{86.5} & 68.8          & \textbf{81.51} \\
%                                  & 1-1-4           & 33(x12.7)     & 1.5            & \textbf{C}  & \XSolidBrush  & 84.7             & \textbf{91.4} & 91.1          & 93.2           & 54            & 84.6          & \textbf{70.3} & 81.33           \\ \hline
% \textbf{BinaryBERT}              & 1-1-4           & 16.5(x25.3)   & 1.5            & \textbf{C}  & \XSolidBrush  & 84.2             & 91.2           & 90.9          & 92.3           & 44.4          & 83.3          & 65.3          & 78.8           \\ \hline
% {\textbf{BEBERT}} & 1-1-4           & 49.5(x8.4)    & 4.5            & \textbf{B}  & \Checkmark  & \textbf{84.8}    & 91.2  & 91.5          & 93.4           & \textbf{57.2} & 85.7          & \textbf{74.2} & \textbf{82.57} \\
%                                  & 1-1-4           & 49.5(x8.4)    & 4.5            & \textbf{C}  & \Checkmark  & 84.7             & \textbf{91.4}  & \textbf{91.6} & \textbf{93.8}  & 57            & 85.2          & 73            & 82.39          \\ \hline
% \textbf{BinaryBERT}              & 1-1-4           & 16.5(x25.3)   & 4.5            & \textbf{C}  & \Checkmark  & 84.2             & 91.2           & 91.4          & 93.7           & 53.3          & \textbf{86}   & 71.5          & 81.61          \\ \hline
% \textbf{baseline}                & 32-32-32        & 418           & 22.5           & \textbf{-}  & \textbf{-}  & 84.9             & 91.5           & 92.1          & 93.2           & 59.7          & 86.3          & 72.2          & 82.84          \\ \hline
% \end{tabular}
% }
% \caption{Results on the GLUE development set for ensemble BinaryBERT. Note that there are three KD strategies for BEBERT: A equal to no KD, B represents prediction KD, and C is two-stage KD.}
% \label{table:2}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|l|l|l|lllllll|l}
\hline
\textbf{Method}                   & \textbf{\#Bits} & \textbf{KD} & \textbf{DA} & \textbf{MNLI-m/mm} & \textbf{QQP}  & \textbf{QNLI}  & \textbf{SST-2} & \textbf{CoLA} & \textbf{MRPC} & \textbf{RTE}  & \textbf{Avg.}  \\ \hline
\textbf{BiBERT}                  & 1-1-1           & \textbf{D}  & \XSolidBrush  & 66.1/67.5             & 84.8          & 72.6           & 88.7           & 25.4          & 72.5          & 57.4          & 66.99          \\ 
\textbf{BEBERT}                  & 1-1-1           & \textbf{D}  & \XSolidBrush  & \textbf{75.7/76.6}    & \textbf{84.9} & \textbf{80.7}  & \textbf{90.2}  & \textbf{27.7} & \textbf{75.1} & \textbf{58.6} & \textbf{70.54} \\ \hline
\textbf{BiBERT}                  & 1-1-1           & \textbf{D}  & \Checkmark  & 66.1/67.5             & 84.8          & 76             & 90.9           & 37.8          & 78.8          & 61            & 70.97          \\ 
\textbf{BEBERT}                  & 1-1-1           & \textbf{D}  & \Checkmark  & \textbf{75.7/76.6}    & \textbf{84.9} & \textbf{80.7*} & \textbf{91.8}  & \textbf{42.6} & \textbf{82.4} & \textbf{65.8} & \textbf{74.97} \\ \hline
\textbf{BinaryBERT}              & 1-1-4           & \textbf{C}  & \XSolidBrush  & 83.9/84.2             & 91.2          & 90.9           & 92.3           & 44.4          & 83.3          & 65.3          & 78.8           \\ \hdashline[2.5pt/5pt]
\textbf{BEBERT} & 1-1-4           & \textbf{A}  & \XSolidBrush  & 84.7/84.6             & 91.3         & \textbf{91.2}  & \textbf{93.3}  & 54.4          & \textbf{86.5} & 68.8          & 81.44          \\
                                 & 1-1-4           & \textbf{B}  & \XSolidBrush  & \textbf{84.8}    & 91.2          & \textbf{91.2}  & \textbf{93.3}  & \textbf{54.8} & \textbf{86.5} & 68.8          & \textbf{81.51} \\
                                 & 1-1-4           & \textbf{C}  & \XSolidBrush  & 84.7             & \textbf{91.4} & 91.1           & 93.2           & 54            & 84.6          & \textbf{70.3} & 81.33          \\ \hline
\textbf{BinaryBERT}              & 1-1-4           & \textbf{C}  & \Checkmark  & 83.9/84.2             & 91.2          & 91.4           & 93.7           & 53.3          & \textbf{86}   & 71.5          & 81.61          \\ \hdashline[2.5pt/5pt]
\textbf{BEBERT} & 1-1-4           & \textbf{B}  & \Checkmark  & \textbf{84.8}    & 91.2          & 91.5           & 93.4           & \textbf{57.2} & 85.7          & \textbf{74.2} & \textbf{82.57} \\
                                 & 1-1-4           & \textbf{C}  & \Checkmark  & 84.7             & \textbf{91.4} & \textbf{91.6}  & \textbf{93.8}  & 57            & 85.2          & 73            & 82.39          \\ \hline
\textbf{baseline}                & full-prec.        & \textbf{-}  & \textbf{-}  & 84.9             & 91.5          & 92.1           & 93.2           & 59.7          & 86.3          & 72.2          & 82.84          \\ \hline
\end{tabular}}
\caption{Results on the GLUE development set. Note that there are four KD strategies for BEBERTs: A equal to without KD, B represents prediction KD, C is two-stage KD, and D indicates KD with direction mismatch distillation(DMD) loss; Four kinds of BEBERTs have distinctive properties in terms of DA and \#Bits}
\label{table:1}
\end{table*}

\section{Experimental Results} \label{sec:res}

% This section evaluates our proposed BEBERT on the GLUE benchmark with various NLP tasks. We first introduce the experimental setup in Section \ref{sec: ex setup}. And then, we compare the accuracy and robustness with baseline models in Section \ref{sec: acc rob}. Finally, we also assess the accuracy trend when boosting iterations increase for figuring out the number of binary models for a well-performed ensemble model in Section \ref{sec: boo num}.

\subsection{Experimental Setup} 
\label{sec: ex setup}
We evaluate BEBERT on the GLUE datasets and report the Matthews correlation for CoLA and Accuracy for the rest.

\noindent\textbf{Ensemble BinaryBERT} uses a half-size TernaryBERT \cite{zhang2020ternarybert} with uniform 4-bit quantized activation as the teacher model. We ensemble the models during the ternary weight split process \cite{bai2021binarybert} with diverse KD methods during training. Following \cite{bai2021binarybert}, we adopt DA with one training epoch and perform vanilla training with six epochs. Especially, On MNLI and QQP, we train three epochs on vanilla training and do not adopt DA. 

\noindent\textbf{Ensemble BiBERT} takes full-precision well-trained DynaBERT as the teacher model. We attempt ensemble process w or w/o  Direction-Matching Distillation. Following \cite{qin2022bibert}, training epochs on each task are 50 for CoLA, 20 for MRPC, STS-B, and RTE, 10 for SST-2 and QNLI, and 5 for MNLI and QQP. We also contain DA and vanilla training as ensemble BinaryBERT.

\noindent\textbf{Robustness Evaluation} injects the input perturbation $\Delta x$ in the embedding layer by Gaussian noise with a variance of 0.01 , motivated by \cite{hua2021noise}. Afterward, we measure the $l_2$ norm of the output accuracy averaged by ten sampling rounds.

\subsection{Analysis of Model Accuracy and Robustness} 
\label{sec: acc rob}
The main results on the development set are shown in Table \ref{table:1}. Our binary ensemble BERTs outperforms the baselines consistently. For instance, on CoLA, ensemble BiBERT and BinaryBERT with DA achieves 4.8\% $\uparrow$ and 3.9\% $\uparrow$, respectively. Furthermore, the ensemble method applying to full binary BERT empirically benefits more compared with applying to half-binarized one, denoting the great potential of our approach in extremely low-bit quantized models.

% \footnote{It is noticeable that we do not put the results of MNLI and QQP in Table \ref{table:2}. Our experiment found that the ensemble method is less effective when applied to strong base models fine-tuned by large datasets.} 


Then we compare the accuracy of BEBERT with a variety of state-of-the-art BERTs designed with model compression methods. The results are taken from the original papers, respectively. Firstly, our designs outperform the compressed full-precision models and attain fewer flops, such as our BEBERT w/o DA surpasses the latest miniLM with an accuracy of 1\% $\uparrow$, with an apparent reduction in terms of model size and flops. Moreover, compared with TinyBERT4L with DA, our BEBERT achieves 6\% $\uparrow$ when the amount of parameters is similar. In terms of efficiency, our BEBERT achieves up to 13x and 7.5x saving on FLOPs and model size with incredible accuracy increase. 

\begin{table}[htbp]
\centering
\resizebox{0.42\textwidth}{!}{
\begin{tabular}{l|lll|l||l}
\hline
\textbf{Method}        & \textbf{\begin{tabular}[c]{@{}l@{}}\#Bits\\ (W-E-A)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Size\\ (MB)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}FLOPs\\ (G)\end{tabular}} & \textbf{DA} & \textbf{Avg.}  \\ \hline
\textbf{DynaBERT}     & full-prec.                                                        & 33                                                           & {\color[HTML]{333333} 0.75}                                  & \XSolidBrush  & 77.36          \\
\textbf{DistilBERT6L} & full-prec.                                                        & 264                                                          & 11.3                                                         & \XSolidBrush  & 78.54          \\
\textbf{BinaryBERT}   & 1-1-4                                                             & 16.5                                                         & 1.5                                                          & \XSolidBrush  & 78.8           \\
\textbf{miniLM}       & full-prec.                                                        & 264                                                          & 11.3                                                         & \XSolidBrush  & 80.63          \\
\textbf{BEBERT}       & 1-1-4                                                             & 33                                                           & 1.5                                                          & \XSolidBrush  & \textbf{81.51} \\ \hline
\textbf{TinyBERT4L}   & full-prec.                                                        & 58                                                           & 1.2                                                          & \Checkmark  & 76.51          \\
\textbf{BinaryBERT}   & 1-1-4                                                             & 16.5                                                         & 1.5                                                          & \Checkmark  & 81.61          \\
\textbf{TinyBERT6L}   & full-prec.                                                        & 264                                                          & 11.3                                                          & \Checkmark  & 81.91          \\
\textbf{TernaryBERT}  & 2-2-8                                                             & 28                                                           & 6                                                            & \Checkmark  & 81.91          \\
\textbf{BEBERT}       & 1-1-4                                                             & 49.5                                                         & 1.5                                                          & \Checkmark  & \textbf{82.57} \\ \hline
\textbf{baseline}     & full-prec.                                                        & 418                                                          & 22.5                                                         & \textbf{-}  & 82.84          \\ \hline
\end{tabular}
}
\caption{Comparison with other state-of-the-art methods on development set of GLUE}
\end{table}

To assess the stability improvement of our BEBERTs, we measure the
accuracy fluctuation after injecting noise to the evaluation datasets. As shown in Fig.~\ref{fig:4}, to evaluate the accuracy fluctuation, we plot the standard deviation bars of BinaryBERT, BiBERT baseline, and our BEBERTs in GLUE datasets. The evaluation shows that BEBERTs, orthogonal to DA, can reduce the output deviation and bias simultaneously.
% the robustness of our BEBERTs with Adaboost can reduce the output deviation and bias simultaneously. Also, data augmentation can contribute to models' robustness.

\begin{figure}[htbp]  
\centering  
\includegraphics[width=0.82\linewidth]{./figs/Robustness.png}
\caption{Robustness analysis for BEBERT with DA in different KD methods. \textbf{Left}: ensemble BinaryBERT training with prediction and 2-stage KD compared with the origin. \textbf{Right}: ensemble BiBERT} 
\label{fig:4} 
\end{figure}

\subsection{Analysis of Boosting Iterations} 
\label{sec: boo num}
To figure out the number of ensemble models required for better performance, we analyze the trend of the accuracy increment of BEBERT w/o DA as the number of boosting iterations increases in Fig.~\ref{fig:5}. 
Interestingly, although ensemble BiBERT performs better at five boosting iterations for all GLUE datasets, ensemble BinaryBERT has a more stable trend and already achieves desirable performance at the boosting iteration of two. 
A possible explanation is that weaker classifiers like BiBERT have many more wrong predictions is a reason for the more fluctuated accuracy trend for ensemble BiBERT. Since AdaBoost relies on the previous classifier's predictions to uplift the weights of the wrongly predicted data for training the next. Moreover, our extra experiment shows that the sample weights for the training set on each iteration of ensemble BiBERT constantly change more than ensemble BinaryBERT.  
As a result, the competence of BEBERT demonstrates a promising path for stable binary BERT models to further develop their performance by ensemble techniques without sacrificing the areas too much.

\begin{figure}[htbp]  
\centering  
\includegraphics[width=0.82\linewidth]{./figs/iteration.png}
\caption{Boosting iterations Analysis for BEBERT w/o DA. }
\label{fig:5} 
\end{figure}
